Translating Large-Scale C Repositories to Idiomatic Rust

Existing C to Rust translation techniques fail to balance quality and scalability: transpilation-based approaches scale to large projects but produce code with poor safety, idiomaticity, and readability. In contrast, LLM-based techniques are prohibitively expensive due to their reliance on frontier models (without which they cannot reliably generate compilable translations), thus limiting scalability. This paper proposes Rustine, a fully automated pipeline for effective and efficient repository-level C to idiomatic safe Rust translation. Evaluating on a diverse set of 23 C programs, ranging from 27 to 13,200 lines of code, Rustine can generate fully compilable Rust code for all and achieve 87% functional equivalence (passing 1,063,099 assertions out of 1,221,192 in test suites with average function and line coverage of 74.7% and 72.2%). Compared to six prior repository-level C to Rust translation techniques, the translations by Rustine are overall safer (fewer raw pointers, pointer arithmetic, and unsafe constructs), more idiomatic (fewer Rust linter violations), and more readable. When the translations cannot pass all tests to fulfill functional equivalence, human developers were able to complete the task in 4.5 hours, on average, using Rustine as debugging support.

==> Algorithms/debugging.tex <==
\SetKwProg{Fn}{Function}{}{}
\caption{\small Automated Debugging Loop}
\label{alg:llm-debug}
\DontPrintSemicolon
\SetAlgoLined

\KwInputs{Rust Project $P$, Rust Test Suite $T$}


  $\textit{commented}\gets[\,]$; change dir to $P$\;

  \While{true}{
    \_,\_,rc $\gets$ \textsc{Build}$(P)$;\\
    $S$, stderr, rc $\gets$ \textsc{RunAndTrace}$(E)$;\\
    \uIf{$rc=0$}{break}
    (f,tag) $\gets$ \textsc{DisableFailingTest}(stderr);\\
    append (f,tag) to $\textit{commented}$
  }

  $i\gets0$; $WL\gets\{\}$\;

  \While{$i < |\textit{commented}|$}{
    uncomment $\textit{commented}[i]$;\\
    $S$, stderr, rc $\gets$ \textsc{RunAndTrace}$(E)$;\\
    \uIf{$rc=0$}{$i\gets i+1$; continue}

    sus $\gets$ \textsc{SuspectsFromTrace}$(S,WL,3)$;\\
    prepare prompt with C code, Rust code, stderr;\\
    resp $\gets$ LLM(prompt); apply edits;\\
    rc $\gets$ \textsc{Build}$(P)$;\\
    \uIf{$rc\neq0$}{revert edits; disable test again}
    \ElseIf{run $E$ fails}{disable test again}
    \Else{add last $S$ element to $WL$}
    $i\gets i+1$
  }

\Fn{\textsc{Build}$(P)$}{
   run \texttt{cargo build}; return (rc, stderr, stdout)
}

\Fn{\textsc{RunAndTrace}$(E)$}{
  execute $E$; extract call stack $S$, stderr, and return code $rc$
}

\Fn{\textsc{DisableFailingTest}$(stderr)$}{
  locate failing line/test from \texttt{stderr} and comment it out,
  return $(file,tag)$
}

\Fn{\textsc{SuspectsFromTrace}$(S,WL,k)$}{
  from end of $S$, collect up to $k$ functions not in whitelist $WL$
}



==> Algorithms/proof.tex <==
We assume all pointer operations in \(f\) are \textbf{well-defined} under the C standard (no undefined behavior, valid bounds).

\begin{definition}[Pointer State $S$]
A pointer state $S(f) = (P_g, P_l)$ for a function $f$ consists of:
\begin{itemize}
    \item $P_g$: a list of pointers defined in the global scope.
    \item $P_l$: a list of local pointers in $f$.
\end{itemize}
\end{definition}

\begin{definition}[Tuple State $T$]
A tuple state $T(f) = (P_g, P_l')$ for a function $f$ consists of:
\begin{itemize}
    \item $P_g$: a list of pointers defined in the global scope.
    \item $P_l'$: a list of tuples $(p_i, \mathit{idx}_i)$ for local pointers in $f$, where $p_i$ is a base pointer and $\mathit{idx}_i$ is its corresponding index.
\end{itemize}
\end{definition}

\begin{definition}[Equivalence of States $S \equiv T$]
A pointer state $S = (P_g, P_l)$ is equivalent to a tuple state $T = (P_g', P_l')$, denoted $S \equiv T$, if:
\begin{itemize}
    \item $P_g = P_g'$ (global pointers are identical).
    \item For every $p_i \in P_l$, there exists a corresponding tuple $(p_i', \mathit{idx}_i) \in P_l'$ such that $p_i = p_i' + \mathit{idx}_i$ (i.e., the effective pointer values match, assuming unit-sized elements for simplicity).
\end{itemize}
\end{definition}

\begin{definition}[Operator $\eta$]
The operator $\eta(p, c) = p'$ applies an arithmetic operation (e.g., addition or subtraction) to pointer $p$ with constant $c$, yielding a new pointer value $p'$.
\end{definition}

\begin{definition}[Tuple $(p, \mathit{idx})$]
The tuple $(p, \mathit{idx})$ represents the effective pointer $p + \mathit{idx}$.
\end{definition}

\begin{definition}[Operator $\eta'$]
The operator $\eta'((p, \mathit{idx}), c) = (p, \mathit{idx}')$ applies an arithmetic operation to the index $\mathit{idx}$ with constant $c$, yielding $\mathit{idx}'$, while keeping the base pointer $p$ unchanged.
\end{definition}

\begin{definition}[Operator $\Gamma$]
The operator $\Gamma(p) = v$ dereferences pointer $p$, returning the value $v$ at the memory location it points to.
\end{definition}

\begin{definition}[Operator $\Gamma'$]
The operator $\Gamma'((p, \mathit{idx})) = v$ dereferences the effective pointer $p + \mathit{idx}$, returning the value $v$ at that memory location.
\end{definition}

\begin{definition}[Operator $\Theta$]
The operator $\Theta(p) = a$ returns the memory address $a$ that pointer $p$ holds (i.e., the value of $p$).
\end{definition}

\begin{definition}[Operator $\Theta'$]
The operator $\Theta'((p, \mathit{idx})) = a$ returns the memory address $a = \&(p[\mathit{idx}])$ (i.e., the effective address of the tuple).
\end{definition}

\begin{definition}[Operator $R$]
The operator $R(p_1, p_2)$ assigns the value of $p_2$ to $p_1$, i.e., $\Theta(p_1) \gets \Theta(p_2)$.
\end{definition}

\begin{definition}[Operator $R'$]
The operator $R'((p_i, \mathit{idx}_i), (p_j, \mathit{idx}_j)) = R(p_i, p_j + \mathit{idx}_j) \cup (\mathit{idx}_i \gets 0)$ assigns the effective value of $(p_j, \mathit{idx}_j)$ to $p_i$ and resets $\mathit{idx}_i$ to 0.
\end{definition}

\begin{definition}[Transformation $\Omega$]
The transformation $\Omega(f) = f'$ on a C function $f$ with pointer state $S(f) = (P_g, P_l)$ is defined as follows:
\begin{itemize}
    \item For every $p_i \in P_l$ where $\eta$ is applied to $p_i$ in $f$, introduce a local variable $\mathit{idx}_i \gets 0$ in $f'$.
    \item For every $p_i \in P_l$, replace $\eta(p_i, c)$ with $\eta'((p_i, \mathit{idx}_i), c)$.
    \item For every $p_i \in P_l$, replace $\Gamma(p_i)$ with $\Gamma'((p_i, \mathit{idx}_i))$.
    \item For every $p_i \in P_l$, replace $\Theta(p_i)$ with $\Theta'((p_i, \mathit{idx}_i))$.
    \item For every assignment $R(p_i, p_j)$, replace it with $R'((p_i, \mathit{idx}_i), (p_j, \mathit{idx}_j))$.
\end{itemize}
The transformation applies only to local pointers in $P_l$; global pointers and non-pointer operations remain unchanged.
\end{definition}

\begin{definition}[Semantics-Preserving Transformation]
A transformation $T(f) = f'$ is semantics-preserving if, under the same initial memory and inputs:
\begin{itemize}
    \item The initial state satisfies $S(f) \equiv T(f')$.
    \item The termination state satisfies $S(f) \equiv T(f')$.
    \item The memory accesses and side effects (e.g., reads/writes) are equivalent.
\end{itemize}
\end{definition}

\begin{proof}
We prove this by structural induction over the statements in $f$, assuming $f$ is a sequence of statements. Let $S_0 \equiv T_0$ be the initial states of $f$ and $f'$, where each transformed local pointer $p_i$ in $f$ corresponds to $(p_i, 0)$ in $f'$.

\textbf{Base case}: Empty function (no statements). Trivially, termination states match initial states, so $S_0 \equiv T_0$.

\textbf{Inductive hypothesis}: Assume that after $k$ statements, the states satisfy $S_k \equiv T_k$, and all prior memory accesses are equivalent.

\textbf{Inductive step}: Consider the $(k+1)$-th statement in $f$, and show $S_{k+1} \equiv T_{k+1}$ with equivalent accesses.

\begin{enumerate}
    \item \textbf{Initialization of indices}: The first step of $\Omega$ introduces $\mathit{idx}_i = 0$ for relevant $p_i \in P_l$. This has no effect on pointers or memory, preserving $S_k \equiv T_k$.
    
    \item \textbf{Arithmetic ($\eta$)}: Replacing $\eta(p_i, c) = p_i'$ with $\eta'((p_i, \mathit{idx}_i), c) = (p_i, \mathit{idx}_i')$. By definition, $p_i' = p_i + \mathit{idx}_i + c = p_i + \mathit{idx}_i'$, so effective pointers match. No memory access occurs.
    
    \item \textbf{Dereference ($\Gamma$)}: Replacing $\Gamma(p_i) = v$ with $\Gamma'((p_i, \mathit{idx}_i)) = v$. By equivalence, $p_i = p_i + \mathit{idx}_i$ only if $\mathit{idx}_i = 0$ initially, but after arithmetic, the effective address is $p_i + \mathit{idx}_i$, so $\Gamma(p_i) = \Gamma'((p_i, \mathit{idx}_i))$. Memory read is identical.
    
    \item \textbf{Address-of ($\Theta$)}: Replacing $\Theta(p_i) = a$ with $\Theta'((p_i, \mathit{idx}_i)) = a$. Similarly, $a = p_i = p_i + \mathit{idx}_i$ (effective address matches). No memory access.
    
    \item \textbf{Assignment ($R$)}: Replacing $R(p_i, p_j)$ with $R'((p_i, \mathit{idx}_i), (p_j, \mathit{idx}_j))$, which sets $p_i \gets p_j + \mathit{idx}_j$ and $\mathit{idx}_i \gets 0$. The effective value assigned to $p_i$ matches the original (since $p_j = p_j + \mathit{idx}_j$ under equivalence), and resetting $\mathit{idx}_i$ prepares for future arithmetic without affecting current state equivalence. No unintended memory access.
\end{enumerate}

Global pointers $P_g$ are unchanged. Non-pointer statements are identical. By induction, termination states satisfy $S_t \equiv T_t$, and all accesses are equivalent. Thus, $\Omega$ preserves semantics.
\end{proof}


==> Listings/downcast.tex <==
\begin{minipage}{.46\linewidth}
\begin{minted}[frame=lines,framesep=1.1mm,baselinestretch=0.47, fontsize=\scriptsize,
        breaklines, breakanywhere, linenos,numbersep=2pt,
        highlightlines={4}]{c}
         ---------- C SOURCE ----------
avlnode *avl_find(avltree *avlt, void *data) {
    ...
    cmp = avlt->compare(data, p->data);
    ...
}
    \end{minted}
    \vspace{-8pt}
\begin{minted}[frame=lines,framesep=1.1mm,baselinestretch=0.47, fontsize=\scriptsize,
    breaklines, breakanywhere, linenos,numbersep=2pt,
    highlightlines={4,5}]{rust}
    ---------- RUSTINE TRANSLATION ----------
pub fn avl_find<'a>(avlt: &'a AvlTree, data: &dyn std::any::Any) -> Option<&'a AvlNode> {
    ...
    let cmp = avlt.compare.as_ref()?.
        as_ref()(data, p.data.as_ref()?);
    ...
}
\end{minted}
\end{minipage}\hfill
\begin{minipage}{.49\linewidth}
\begin{minted}[frame=lines,framesep=1mm,baselinestretch=0.47, fontsize=\scriptsize,
    breaklines, breakanywhere, linenos,numbersep=2pt,
    highlightlines={5-10}]{rust}
    ---------- MANUAL DEBUGGED CODE ----------

pub fn avl_find<'a>(avlt: &'a AvlTree, data: Option<&Mydata>) -> Option<&'a AvlNode> {
    ...

    let cmp = (avlt.compare)(
        data,
        p.data.as_ref().map(|data| {
            data.downcast_ref::<Mydata>().expect("Failed")
            }),
    );

    ...
}
\end{minted}
\end{minipage}\hfill

==> Listings/qsortdebug.tex <==
\begin{minipage}{.48\linewidth}
    % --- C Source ---
    \begin{minted}[frame=lines,framesep=1mm,baselinestretch=0.47, fontsize=\scriptsize,
        breaklines, breakanywhere, linenos,numbersep=2pt,
        highlightlines={8,11}]{c}
              -- qsort Source Code in C --
int partition(int arr[], int low, int high) {
  int pivot = arr[high];
  int i = low - 1;
  for (int j = low; j <= (high - 1); j += 1) {
    if (arr[j] <= pivot) {
      i += 1;
      swap(&arr[i], &arr[j]);
    }
  }
  swap(&arr[i + 1], &arr[high]);
  return i + 1;
}
    \end{minted}
    \vspace{-6pt}
    % --- Rustine Translation ---
    \begin{minted}[frame=lines,framesep=1mm,baselinestretch=0.47, fontsize=\scriptsize,
        breaklines, breakanywhere, linenos,numbersep=2pt,
        highlightlines={8-9,13-14}]{rust}
             -- Rustine Translation --
pub fn partition(arr: &mut [i32], low: usize, high: usize) -> usize {
  let pivot = arr[high];
  let mut i = low as i32 - 1;
  for j in low..high {
    if arr[j] <= pivot {
      i += 1;
      let (a, b) = arr.split_at_mut(j);
      swap(&mut a[i as usize], &mut b[0]);
    }
  }
  let final_pos = (i + 1) as usize;
  let (a, b) = arr.split_at_mut(high);
  swap(&mut a[final_pos], &mut b[0]);
  final_pos
}
    \end{minted}
\end{minipage}\hspace{0.01\linewidth}
\begin{minipage}{.48\linewidth}
    % --- Rustine Debug ---
    \begin{minted}[frame=lines,framesep=1mm,baselinestretch=0.47, fontsize=\scriptsize,
        breaklines, breakanywhere, linenos,numbersep=2pt,
        highlightlines={12-16,20-24}]{rust}
              -- Rustine Debugging --
pub fn partition(arr: &mut [i32], low: usize, high: usize) -> usize {
  if arr.is_empty() || low > high || high >= arr.len() {
    panic!("Invalid array bounds in partition");
  }
  let pivot = arr[high];
  let mut i = low as i32 - 1;
  for j in low..high {
    if arr[j] <= pivot {
      i += 1;
      let i_usize = i as usize;
      if i_usize < j {
        let (left, right) = arr.split_at_mut(j);
        swap(&mut left[i_usize], &mut right[0]);
      }
      // if i_usize == j, no swap needed
    }
  }
  let final_pos = (i + 1) as usize;
  if final_pos < high {
    let (left, right) = arr.split_at_mut(high);
    swap(&mut left[final_pos], &mut right[0]);
  }
  // If final_pos == high, no swap needed
  final_pos
}
    \end{minted}
\end{minipage}

==> Tables/Ablation-Pointer.tex <==

\setlength{\tabcolsep}{6pt} 
\renewcommand{\arraystretch}{1.1} 

\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
\multirow{2}{*}{\textbf{ID}} & \multirow{2}{*}{\textbf{Subject}}
& \multicolumn{3}{c|}{\textbf{Pointers}}
& \multicolumn{3}{c}{\textbf{Unsafe Constructs}} \\ \cline{3-8}
& & \textbf{Pointer Arithmetic} & \textbf{RP Declarations} & \textbf{RP Dereferences}
& \textbf{Lines} & \textbf{Type Casts} & \textbf{Calls} \\ \hline

3 & rgba &
0 & 0 & 0 &
0 & 0 & 0\\ 

6 & grabc &
0 & 15 & 8 &
224 & 29 & 101 \\ 

7 & urlparser &
10 & 6 & 9 &
48 & 7 & 28 \\

8 & xzoom &
21 & 21 & 17 &
457 & 59 & 283 \\

9 & genann &
21 & 5 & 16 &
52 & 16 & 37 \\

10 & ht &
1 & 1 & 0 &
40 & 0 & 32 \\ 

12 & libcsv &
4 & 6 & 8 &
107 & 2 & 40 \\

14 & libopenaptx &
8 & 2 & 2 &
9 & 2 & 6 \\ 

15 & libtree &
16 & 13 & 5 &
184 & 31 & 152 \\ 

16 & opl &
18 & 2 & 3 &
20 & 1 & 12 \\ 

17 & libzahl &
15 & 6 & 4 &
1700 & 5 & 703 \\ 

18 & zopfli &
48 & 10 & 23 &
81 & 8 & 45 \\

19 & snudown &
4 & 16 & 34 &
158 & 51 & 96 \\ 

20 & lodepng &
116 & 33 & 25 &
157 & 17 & 62\\ 

21 & bzip2 &
11 & 62 & 42 &
1069 & 149 & 567\\ 

22 & binn &
50 & 108 & 55 &
629 & 248 & 536\\ 

23 & tulpindicator &
45 & 42 & 88 &
894 & 90 & 455\\ \hline


\multicolumn{2}{c|}{\textbf{Average}} 
& 22.82 & 20.47 & 19.94   
& 342.88 & 42.06 & 185.59 \\ \hline   
\end{tabular}
